Joint Denoising / Compression of Image Contours via Shape Prior and Context Tree

With the advent of depth sensing technologies, the extraction of object contours in images---a common and important pre-processing step for later higher-level computer vision tasks like object detection and human action recognition---has become easier. However, acquisition noise in captured depth images means that detected contours suffer from unavoidable errors. In this paper, we propose to jointly denoise and compress detected contours in an image for bandwidth-constrained transmission to a client, who can then carry out aforementioned application-specific tasks using the decoded contours as input. We first prove theoretically that in general a joint denoising / compression approach can outperform a separate two-stage approach that first denoises then encodes contours lossily. Adopting a joint approach, we first propose a burst error model that models typical errors encountered in an observed string y of directional edges. We then formulate a rate-constrained maximum a posteriori (MAP) problem that trades off the posterior probability p(x'|y) of an estimated string x' given y with its code rate R(x'). We design a dynamic programming (DP) algorithm that solves the posed problem optimally, and propose a compact context representation called total suffix tree (TST) that can reduce complexity of the algorithm dramatically. Experimental results show that our joint denoising / compression scheme outperformed a competing separate scheme in rate-distortion performance noticeably.

==> alternative.tex <==
In this section, we show that it is possible to formulate an alternative \textit{rate-constrained Maximum Likelihood (ML)} problem or \textit{unconstrained Maximum a Posterior (MAP)} problem by combining the prior term and the rate term into a \textit{super rate} term denoted by $R_s(\hat{\vec{x}})$ or a \textit{super prior} denoted by $P_s(\hat{\vec{x}})$ respectively.
\red{I don' get this super rate and super prior. why do we need this definitions? this needs more explanation why these combos are reasonable.}
The corresponding formulations are as follows:
\begin{equation}
\label{eq:alternative_lagrangian_objective}
\underset{\hat{\vec{x}}\in  \mathcal{S}}{\min}\ -\log P(\vec{y}|\hat{\vec{x}})+\lambda_s R_s(\hat{\vec{x}})
\end{equation}
\begin{equation}
\label{eq:alternative_MAP}
\underset{\hat{\vec{x}}\in  \mathcal{S}}{\max}\ P(\vec{y}|\hat{\vec{x}})\cdot P_s(\hat{\vec{x}})
\end{equation}
Different from (\ref{eq:lagrangian_objective}), (\ref{eq:alternative_lagrangian_objective}) performs the rate-constrained ML estimation, \textit{i.e.}, find $\hat{\vec{x}} \in  \mathcal{S}$ that maximize likelihood $P(\vec{y}|\hat{\vec{x}})$ subject to $R_s(\hat{\vec{x}})\leq R_{\max}$.
In contrast, (\ref{eq:alternative_MAP}) performs the unconstrained MAP estimation, \textit{i.e.}, find $\hat{\vec{x}} \in  \mathcal{S}$ that maximizes the product of the likelihood $P(\vec{y}|\hat{\vec{x}})$ and the super prior $P_s(\hat{\vec{x}})$.

In (\ref{eq:objective}), both the prior term and the rate term can be regarded as a modelling of the contour signal.
Specifically, the prior models the underlying statistics of the contour by assuming that contours are more likely to be straight than curvy, which is independent of the signal observations. 
In contrast, the rate term models the symbol probabilities from the training data, which is a data-driven statistical model.
It is possible to combine the two terms into one term as in (\ref{eq:alternative_lagrangian_objective}) and (\ref{eq:alternative_MAP}), but in general they are capturing distinct distributions of the contour.
For example, if the rate constraint is loose and the signal is corrupted by heavy noise, then the reconstructed contours obtained by solving (\ref{eq:objective}) without the prior term are not likely straight.
Similarly, after removing the rate term in (\ref{eq:objective}), the reconstructed contours may not have a small entropy (rate).
\red{point being made here is not crystal clear.}

To find out the relationship between the rate-constrained MAP, rate-constrained ML and unconstrained MAP problems, we rewrite (\ref{eq:alternative_MAP}) as follows:
\begin{equation}
\underset{\hat{\vec{x}}\in  \mathcal{S}}{\min}\ -\log P(\vec{y}|\hat{\vec{x}}) - \beta_s \log P_s(\hat{\vec{x}})
\end{equation}
When the combined super rate term and super prior term are both equal to the sum of the prior term and rate term in the original formulation (\ref{eq:objective}), \textit{i.e.}, 
\begin{equation}
\lambda_s R_s(\hat{\vec{x}}) = -\beta_s \log P_s(\hat{\vec{x}}) = \lambda R(\hat{\vec{x}}) - \beta \log P(\hat{\vec{x}}),
\end{equation}
all the three formulations lead to the same solution.
This provides additional insight into the relationship between the rate-constrained MAP, rate-constrained ML and unconstrained MAP problems.
\red{Idon't get this. why do we have this discussion?}
